Targeting Multi-Loop Integrals with Neural Networks

Numerical evaluations of Feynman integrals often proceed via a deformation of the integration contour into the complex plane. While valid contours are easy to construct, the numerical precision for a multi-loop integral can depend critically on the chosen contour. We present methods to optimize this contour using a combination of optimized, global complex shifts and a normalizing flow. They can lead to a significant gain in precision.

==> incl_coupling.tex <==

\definecolor{Gcolor}{HTML}{2c7fb8}
\definecolor{Dcolor}{HTML}{f03b20}

\tikzset{fontscale/.style = {font=\relsize{#1}}
}

\tikzstyle{Data} = [thick, rectangle, minimum width=0.75cm, minimum height=0.75cm,text centered, draw=black]
\tikzstyle{Network} = [thick, rectangle, rounded corners, minimum width=1cm, minimum height=0.67cm,text centered, draw=black, fill=black, opacity=0.8]
\tikzstyle{Operation} = [thick, circle, minimum width=0.9cm, minimum height=0.75cm,text centered, draw=black, fill=black, opacity=0.8]

\tikzstyle{io} = [circle, text centered, draw=black, minimum width=0.75cm]

\tikzstyle{Connection} = [thick, circle, inner sep = 1.5pt, text centered, fill=black]



\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{tikzpicture}[node distance=1.5cm]


\node (v1) [Data] {$y_1$};

\node (Add1) [Operation, left of = v1, xshift=-0.25cm, text=white] {+};
\node (Mult1) [Operation, left of = Add1, xshift=0.25cm, text=white] {$\bigodot$};



\node (Mult2) [Operation, right of = v1, xshift=0.5cm, text=white, yshift=-2.5cm] {$\bigodot$};
\node (Add2) [Operation, right of = Mult2, xshift=-0.25cm, text=white] {+};


\node (u1) [Data, left of = Mult1, xshift=-1cm] {$x_1$};
\node (u2) [Data, below of = u1, yshift=-1cm] {$x_2$};
\node (v2) [Data, right of = Add2] {$y_2$};


\node (s1) [Network, below of = Mult1, xshift=-0.5cm, yshift=0.25cm, text=white] {$s_1$};
\node (t1) [Network, below of = Add1, xshift=-0.5cm, yshift=0.25cm, text=white] {$t_1$};
\node (s2) [Network, above of = Mult2, xshift=-0.5cm, yshift=-0.25cm, text=white] {$s_2$};
\node (t2) [Network, above of = Add2, xshift=-0.5cm, yshift=-0.25cm, text=white] {$t_2$};


\node (conn1) [Connection, left of = s1, xshift=-2cm] {};
\node (conn2) [Connection, right of = t2, xshift=2cm] {};
\node (conn3) [Connection, below of = s1, yshift=0.25cm, xshift=-0.55cm] {};
\node (conn4) [Connection, below of = t1, yshift=0.25cm, xshift=-0.55cm] {};
\node (conn5) [Connection, above of = s2, yshift=-0.25cm, xshift=-0.55cm] {};
\node (conn6) [Connection, above of = t2, yshift=-0.25cm, xshift=-0.55cm] {};

\node (in) [io, left of = conn1, xshift=0.25cm] {in};
\node (out) [io, right of = conn2, xshift=-0.25cm] {out};

\coordinate[ above of = v2, yshift=1.0cm] (C1);

%\coordinate[ above of = xrecon, xshift=0cm, yshift=0.75cm] (Lin2);

\draw [color=black] ([yshift=0em]conn1.center) -- (u1.west);
\draw [color=black] ([yshift=0em]u1.east) -- (Mult1.west);
\draw [color=black] ([yshift=0em]Mult1.east) -- (Add1.west);
\draw [color=black] ([yshift=0em]Add1.east) -- (v1.west);
\draw [color=black] ([yshift=0em]v1.east) -- (conn5.center);
\draw [color=black] ([yshift=0em]conn5.center) -- (conn6.center);
\draw [color=black] ([yshift=0em]conn6.center) -- (C1);
\draw [color=black] ([yshift=0em]C1) -- (conn2.center);

\draw [color=black] ([yshift=0em]conn1.center) -- (u2.west);
\draw [color=black] ([yshift=0em]u2.east) -- (conn3.center);
\draw [color=black] ([yshift=0em]conn3.center) -- (conn4.center);
\draw [color=black] ([yshift=0em]conn4.center) -- (Mult2.west);
\draw [color=black] ([yshift=0em]Mult2.east) -- (Add2.west);
\draw [color=black] ([yshift=0em]Add2.east) -- (v2.west);
\draw [color=black] ([yshift=0em]v2.east) -- (conn2.center);

\draw [arrow, color=black] ([yshift=0em]in.east) -- (conn1.west);
\draw [arrow, color=black] ([yshift=0em]conn2.center) -- (out.west);

%\draw [color=black] ([yshift=0em]conn3.center) -- (Mult1.south);
%\draw [color=black] ([yshift=0em]conn4.center) -- (Add1.south);

\draw [color=black] ([yshift=0em]conn3.center) -- ([xshift=-0.075cm]s1.south);
\draw [color=black] ([yshift=0em]conn4.center) -- ([xshift=-0.075cm]t1.south);
\draw [color=black] ([xshift=0.275cm]s1.north) -- (Mult1.south);
\draw [color=black] ([xshift=0.275cm]t1.north) -- (Add1.south);

\draw [color=black] ([yshift=0em]conn5.center) -- ([xshift=-0.075cm]s2.north);
\draw [color=black] ([yshift=0em]conn6.center) -- ([xshift=-0.075cm]t2.north);
\draw [color=black] ([xshift=0.275cm]s2.south) -- (Mult2.north);
\draw [color=black] ([xshift=0.275cm]t2.south) -- (Add2.north);


%\draw [arrow, dotted, color=black] ([yshift=0em]Loss.south) -- ([yshift=0em]Bottleneck.north);


\end{tikzpicture}

